AFLoRA: Adaptive Federated Fine-Tuning of Large Language Models with Resource-Aware Low-Rank Adaption

Federated fine-tuning has emerged as a promising approach to adapt foundation models to downstream tasks using decentralized data. However, real-world deployment remains challenging due to the high computational and communication demands of fine-tuning Large Language Models (LLMs) on clients with data and system resources that are heterogeneous and constrained. In such settings, the global model's performance is often bottlenecked by the weakest clients and further degraded by the non-IID nature of local data. Although existing methods leverage parameter-efficient techniques such as Low-Rank Adaptation (LoRA) to reduce communication and computation overhead, they often fail to simultaneously ensure accurate aggregation of low-rank updates and maintain low system costs, thereby hindering overall performance. To address these challenges, we propose AFLoRA, an adaptive and lightweight federated fine-tuning framework for LLMs. AFLoRA decouples shared and client-specific updates to reduce overhead and improve aggregation accuracy, incorporates diagonal matrix-based rank pruning to better utilize local resources, and employs rank-aware aggregation with public data refinement to strengthen generalization under data heterogeneity. Extensive experiments demonstrate that AFLoRA outperforms state-of-the-art methods in both accuracy and efficiency, providing a practical solution for efficient LLM adaptation in heterogeneous environments in the real world.

==> Evaluation-old.tex <==
\section{Performance Evaluation}\label{sec:evaluation}
\begin{figure*}[!t]
\centering
\label{fig:ablation}
\subfigure[GPT-2]{\label{fig:ablation_gpt}
\includegraphics[width=0.625\columnwidth]{pic/ablation_gpt.pdf}
}
\subfigure[TinyLlama-1.1B]{\label{fig:ablation_llama}
\includegraphics[width=0.625\columnwidth]{pic/ablation_llama.pdf}
}
\subfigure[Qwen2.5-3B]{\label{fig:ablation_qwen}
\includegraphics[width=0.625\columnwidth]{pic/ablation_qwen.pdf}
}
\vspace{-2mm}
\caption{Effect of the proposed mechanisms.}
\label{fig:Ablation}
\vspace{-4mm}
\end{figure*}


\begin{table}[!t]
\centering
\caption{Cost comparison of AFLoRA and AFLoRA w/o DDR on different foundation models and datasets.}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{\makecell{Foundation \\ Model}}} & \multirow{2}{*}{\textbf{\makecell{Dataset}}} & \multicolumn{2}{c}{\textbf{Computation/Communication Cost}}\\
\cline{3-4}
 & & \textbf{AFLoRA} & \textbf{AFLoRA w/o DDR}\\
\midrule
\multirow{2}{*}{\textbf{GPT-2}} 
& \textbf{Wizard}   &\textbf{0.0073/0.0072} &0.0095/0.0085  \\
& \textbf{Dolly}   &\textbf{0.0060/0.0060} &0.0095/0.0085 \\
& \textbf{FinGPT}   &\textbf{0.0072/0.0072} &0.0095/0.0085  \\
& \textbf{AG News}   &\textbf{0.0081/0.0079} &0.0095/0.0085 \\
\midrule
\multirow{2}{*}{\textbf{TinyLlama-1.1B}} 
& \textbf{Wizard}   &\textbf{/} &/  \\
& \textbf{Dolly}   &\textbf{/} &/ \\
& \textbf{FinGPT}   &\textbf{/} &/  \\
& \textbf{AG News}   &\textbf{/} &/ \\
\midrule
\multirow{2}{*}{\textbf{Qwen2.5-3B}} 
& \textbf{Wizard}   &\textbf{0.0050/0.0050} &0.0062/0.0061  \\
& \textbf{Dolly}   &\textbf{0.0056/0.0056} &0.0062/0.0061 \\
& \textbf{FinGPT}   &\textbf{0.0040/0.0040} &0.0062/0.0061  \\
& \textbf{AG News}   &\textbf{0.0062/0.0061} &\textbf{0.0062/0.0061} \\
\bottomrule
\end{tabular}
\label{Table:ablation}
\end{table}

\begin{itemize}
    \item \textbf{WizardLM} \cite{wizard} is a conversational dataset comprising approximately 250,000 instruction-response pairs.%, designed to evaluate LLMs on complex instruction-following and question-answering tasks. %It is randomly and evenly distributed across 10 clients to serve as the general dataset under the IID setting. 
    \item \textbf{FinGPT-Sentiment} \cite{fingpt} is a dataset for financial sentiment analysis, containing over 10,000 annotated entries curated from financial news and social media sources. %It is also randomly and evenly distributed across 10 clients to serve as the domain dataset under the IID setting.
    \item \textbf{Databricks-Dolly-15k} \cite{dolly} is a high-quality human-generated instruction-following dataset, consisting of 15,000 samples across diverse tasks including open-domain QA, classification, and summarization. %Following the Non-IID partitioning strategy described in FedIT\cite{fedit}, it is distributed to 10 clients to form the general dataset under the Non-IID setting. The smaller the value of $\epsilon$, the higher the Non-IID degree.
    \item \textbf{AG News} \cite{agnews} is a benchmark for news classification, containing over 1.2 million articles categorized into four domains (World, Sports, Business, and Sci/Tech). %To construct the domain dataset under the Non-IID setting, it is partitioned using a label-skew scheme, where each client receives data from only two distinct classes.
    \item \textbf{Alpaca} \cite{alpaca} is an instruction-following dataset constructed by Stanford using self-instruct techniques, comprising 52,000 examples spanning a wide range of user prompts and corresponding responses. We randomly select 2\% of the data to form a small public dataset.
\end{itemize}

\begin{table*}[!t]
\centering
\caption{Performance and cost comparison of AFLoRA and baseline methods on general datasets. For both HETLoRA and FlexLoRA, the computation overhead is equal to their respective communication overhead.}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{\makecell{Foundation \\ Model}}} & \multirow{2}{*}{\textbf{\makecell{General\\Dataset}}} & \multicolumn{4}{c|}{\textbf{Model Performance}} & \multicolumn{4}{c}{\textbf{Computation/Communication Cost}}\\
\cline{3-10}
 & & \textbf{AFLoRA} & \textbf{FLoRA} & \textbf{HETLoRA} & \textbf{FlexLoRA}& \textbf{AFLoRA} & \textbf{FLoRA} & \textbf{HETLoRA} & \textbf{FlexLoRA}\\
\midrule
\multirow{2}{*}{\textbf{GPT-2}} 
& \textbf{Wizard}           &\textbf{0.3929}    &0.3752  &0.1967 & 0.2523 &\textbf{0.0073/0.0072} &0.0190/0.0951 &0.0190 &0.0190 \\
& \textbf{Dolly}   &\textbf{0.3685}    &0.3099  &0.2005 & 0.2549 &\textbf{0.0060/0.0060} &0.0190/0.0951 &0.0190 &0.0190\\
\midrule
\multirow{2}{*}{\textbf{TinyLlama-1.1B}} 
& \textbf{Wizard}           &\textbf{0.}    &0.  &0. &0.  &\textbf{0./0.} &0./0. &0. &0. \\
& \textbf{Dolly}   &\textbf{0.}    &0.  &0. & 0. &\textbf{0./0.} &0./0. &0. &0.\\
\midrule
\multirow{2}{*}{\textbf{Qwen2.5-3B}} 
& \textbf{Wizard}           &\textbf{0.5555}    &0.4781  &0.5489 &0.5506  &\textbf{0.0050/0.0050} &0.0123/0.0614 &0.0123 &0.0123 \\
& \textbf{Dolly}   &\textbf{0.6097}    &0.5626  &0.5664 & 0.6015 &\textbf{0.0056/0.0056} &0.0123/0.0614 &0.0123 &0.0123\\
\bottomrule
\end{tabular}
\label{Table:general}
\end{table*}


\begin{table*}[!t]
\centering
\caption{Performance and cost comparison of AFLoRA and baseline methods on domain datasets. For both HETLoRA and FlexLoRA, the computation overhead is equal to their respective communication overhead.}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{\makecell{Foundation \\ Model}}} & \multirow{2}{*}{\textbf{\makecell{General\\Dataset}}} & \multicolumn{4}{c|}{\textbf{Model Performance}} & \multicolumn{4}{c}{\textbf{Computation/Communication Cost}}\\
\cline{3-10}
 & & \textbf{AFLoRA} & \textbf{FLoRA} & \textbf{HETLoRA} & \textbf{FlexLoRA}& \textbf{AFLoRA} & \textbf{FLoRA} & \textbf{HETLoRA} & \textbf{FlexLoRA}\\
\midrule
\multirow{2}{*}{\textbf{GPT-2}} 
& \textbf{FinGPT}   &\textbf{0.6144}    &0.5746  &0.3975 & 0.2523 &\textbf{0.0072/0.0072} &0.0190/0.0951 &0.0190 &0.0190  \\
& \textbf{AG news}            & \textbf{0.3584}       & 0.2900          & 0.2020        &0.2653 &\textbf{0.0081/0.0079} &0.0190/0.0951 &0.0190 &0.0190  \\
\midrule
\multirow{2}{*}{\textbf{TinyLlama-1.1B}} 
& \textbf{FinGPT}   &\textbf{0.}    &0.  &0. & 0. &\textbf{0./0.} &0./0. &0. &0.  \\
& \textbf{AG news}            & \textbf{0.}       &0.           & 0.        &  0. &\textbf{0./0.} &0./0. &0. &0.  \\
\midrule
\multirow{2}{*}{\textbf{Qwen2.5-3B}} 
& \textbf{FinGPT}   &\textbf{0.9209}    &0.9143  &0.8622 & 0.9129 &\textbf{0.0040/0.0040} &0.0123/0.0614 &0.0123 &0.0123  \\
& \textbf{AG news}            & \textbf{0.5504}       &0.4728           & 0.2832        &  0.2500 &\textbf{0.0062/0.0061} &0.0123/0.0614 &0.0123 &0.0123  \\
\bottomrule
\end{tabular}
\label{Table:domain}
\end{table*}


\begin{figure*}[!t]
\centering
\label{fig:noniid}
\subfigure[GPT-2]{\label{fig:noniid_gpt}
\includegraphics[width=0.625\columnwidth]{pic/noniid_gpt.pdf}
}
\subfigure[TinyLlama-1.1B]{\label{fig:noniid_llama}
\includegraphics[width=0.625\columnwidth]{pic/noniid_llama.pdf}
}
\subfigure[Qwen2.5-3B]{\label{fig:noniid_qwen}
\includegraphics[width=0.625\columnwidth]{pic/noniid_qwen.pdf}
}
\vspace{-2mm}
\caption{The performance comparison when the degree of non-IID $\epsilon$ changes.}
\label{fig:noniid}
\vspace{-4mm}
\end{figure*}


In this section, we evaluate the performance and efficiency of AFLoRA to validate its effectiveness. 


\subsection{Setup}


\textbf{Dataset.} 
We conduct experiments on four datasets widely used in federated fine-tuning experiments:

\begin{itemize}
    \item \textbf{WizardLM} \cite{wizard} is a multi-turn conversational dataset comprising approximately 250,000 instruction-response pairs, designed to evaluate large language models on complex instruction-following and question-answering tasks. %It is randomly and evenly distributed across 10 clients to serve as the general dataset under the IID setting. 
    \item \textbf{Databricks-Dolly-15k} \cite{dolly} is a high-quality human-generated instruction-following dataset, consisting of 15,000 samples across diverse tasks including open-domain QA, classification, and summarization. %Following the Non-IID partitioning strategy described in FedIT\cite{fedit}, it is distributed to 10 clients to form the general dataset under the Non-IID setting. The smaller the value of $\epsilon$, the higher the Non-IID degree.
    \item \textbf{FinGPT-Sentiment} \cite{fingpt} is a domain-specific dataset for financial sentiment analysis, containing over 10,000 annotated entries curated from financial news and social media sources. %It is also randomly and evenly distributed across 10 clients to serve as the domain dataset under the IID setting.
    \item \textbf{AG News} \cite{agnews} is a widely used benchmark for news classification, containing over 1.2 million articles categorized into four domains (World, Sports, Business, and Sci/Tech). %To construct the domain dataset under the Non-IID setting, it is partitioned using a label-skew scheme, where each client receives data from only two distinct classes.
    \item \textbf{Alpaca} \cite{alpaca} is an instruction-following dataset constructed by Stanford using self-instruct techniques, comprising 52,000 examples spanning a wide range of user prompts and corresponding responses. We randomly select 2\% of the data to form a small public dataset.
\end{itemize}
For the QA datasets, we report accuracy on the \textbf{MMLU} benchmark \cite{mmlu}, a widely adopted multi-task evaluation suite covering questions from multiple academic and professional fields. For financial sentiment analysis, model performance is assessed using classification accuracy on the FPB\cite{fpb} benchmark. For news classification, performance is computed on the AG News test set\cite{agnews}.

\textbf{Model.} GPT-2\cite{gpt} model (124 M) with LoRA applied to a selected set of modules, specifically c\_attn, c\_proj, and c\_fc, as specified in the lora\_target\_modules configuration. TinyLlama-1.1B\cite{tinyllama} and Qwen2.5-3B\cite{qwen} with lora\_target\_modules setting as q\_proj and v\_proj. 

\textbf{Clients.} Our experiments involve 1 server and 10 clients. Each client is assigned a resource constraint that limits the maximum rank of the LoRA matrices it can fine-tune, set respectively as [64,32,16,16,8,8,4,4,4,4]. When testing performance under different non-IID degrees, 20\% of the clients are selected to participate in training during each epoch. In all other experiments, the client selection ratio is set to 1.

\textbf{Metrics.} We use two metrics to evaluate the effectiveness of the proposed AFLoRA: global model accuracy and the ratio of locally trained or communicated parameters to the total number of parameters in the original LLM.

\textbf{Baseline.}
We compare our method with the following representative baselines for federated LoRA finetuning:

\begin{itemize}
    \item \textbf{FLoRA}\cite{flora} aggregates LoRA parameters by first concatenating the \( \mathbf{B} \) and \( \mathbf{A} \) matrices from all clients, and then multiplying the concatenated \( \mathbf{B} \) and \( \mathbf{A} \) to obtain the global update.

    \item \textbf{HETLoRA}\cite{hetlora} performs zero-padding on the client-specific \( \mathbf{B} \) and \( \mathbf{A} \) matrices to match the maximum rank observed across clients in order to support heterogeneous ranks across clients. The zero-padded matrices are then aggregated and multiplied.

    \item \textbf{FlexLoRA}\cite{flexlora} first computes the reconstructed matrix \( \mathbf{W}_k = \mathbf{B}_k \mathbf{A}_k \) on each client, then applies weighted model averaging to obtain the aggregated \( \mathbf{W} \). The server subsequently performs singular value decomposition (SVD) on \( \mathbf{W} \) to extract a low-rank approximation that is compatible with each client's specified rank.
\end{itemize}

%\begin{table}[!t]
%\centering
%\renewcommand{\arraystretch}{1.3}
%\begin{tabular}{c|c|cc|cc}
%\toprule
%\multirow{2}{*}{\textbf{\makecell{Foundation \\ Model}}} & \multirow{2}{*}{\textbf{\makecell{Finetuning\\Method}}} & \multicolumn{2}{c|}{\textbf{General}} & \multicolumn{2}{c}{\textbf{Domain}} \\
%\cline{3-6}
% & & \textbf{Dolly} & \textbf{Wizard} & \textbf{Fingpt} & \textbf{AG\_news}\\
%\midrule
%\multirow{4}{*}{\textbf{GPT-2}} 
%& \textbf{AFLoRA}   &        & \textbf{0.3929} & \textbf{0.6117} & \\
%& FLoRA            &        & 0.3752          & 0.5322          & \\
%& HETLoRA          &        & 0.1967          & 0.5119          & \\
%& FlexLoRA         &        & 0.2523          & 0.5182          & \\
%\bottomrule
%\end{tabular}
%\caption{Performance comparison of different federated LoRA fine-tuning methods on general and domain-specific tasks.}
%\label{Table:finetune-results}
%\end{table}

%\begin{table}[!t]
%\centering
%\caption{Model performance comparison of AFLoRA and baseline methods on general datasets}
%\renewcommand{\arraystretch}{1.3}
%\begin{tabular}{c|c|cccc}
%\toprule
%\multirow{2}{*}{\textbf{\makecell{Foundation \\ Model}}} & \multirow{2}{*}{\textbf{\makecell{General\\Dataset}}} & \multicolumn{4}{c}{\textbf{Methods}} \\
%\cline{3-6}
% & & \textbf{AFLoRA} & \textbf{FLoRA} & \textbf{HETLoRA} & \textbf{FlexLoRA}\\
%\midrule
%\multirow{2}{*}{\textbf{GPT-2}} 
%& \textbf{Dolly}   &\textbf{0.3685}    &0.3099  &0.1967 & 0.2523\\
%& \textbf{Wizard}           &\textbf{0.3929}    &0.3752  &0.1967 & 0.2523 \\
%\bottomrule
%\end{tabular}
%\label{Table:finetune-results-general}
%\end{table}

\subsection{Evaluation Results}
\subsection{Effect of the proposed mechanisms}
To verify the effectiveness of the proposed Diagonal-Based Dynamic Rank Assignment mechanism (DDR) and Server-Side Heterogeneous Aggregation with Shared Representation Refinement (SHA) mechanism,  we conduct experiments of AFLoRA with and without DDA and SHA, respectively. 
Among them, AFLoRA without DDR initially assigns ranks to each client based on their capabilities and maintains these rank assignments throughout the entire fine-tuning process.
AFLoRA without SHA performs weighted aggregation of client updates proportional to the amount of data used for fine-tuning at each client, without leveraging any public datasets for enhancement.
The performance comparison results are shown in Fig.\ref{fig:Ablation} and Table.\ref{Table:ablation}.

It is shown that not performing the DDR mechanism results in both overall accuracy drop (nearly ??\% on MNIST and ??\% on CIFAR-10) and Cost increase (). 
This is because the DDR mechanism dynamically adjusts client rankings based on the knowledge acquisition patterns of the LoRA-adapted foundation model on local datasets while simultaneously focusing optimization on established effective directions, thereby preventing overfitting of client-specific LoRA adaptations. Furthermore, it selectively retains only the most information-rich dimensions of LoRA updates, thereby reducing both computational and communication resource overhead.
In conclusion, DDR is an indispensable component for AFLoRA. 

We can also observe that SHA enhances the overall accuracy of the global model on different foundation models and datasets.
For example, adopting SHA increases (the overall accuracy by over 30\% on MNIST and the generalization accuracy by almost 20\% on CIFAR-10). 
This demonstrates the effectiveness of the SHA mechanism in boosting AFLoRA's performance. 
SHA enhances model quality by assigning higher aggregation weights to clients with larger ranks, thereby capturing richer local data characteristics. 
It further employs a public data refinement step to prevent the aggregated model from overly biasing toward individual client data distributions, ultimately improving the generalization capability of the global model.



\subsection{Evaluation on General Datasets}
We evaluate the model on the general dataset to assess its performance on standard tasks, measuring the algorithm's overall effectiveness when task relevance is broad and data diversity is high, which is more closely resemble large-scale, real-world applications spanning multiple user tasks.

We compare AFLoRA with baseline methods on general dataset in terms of the global model performance and computation/communication cost, the results are shown in Table.\ref{Table:general}. We can find that AFLoRA's performance outperforms existing methods, which demonstrates the effectiveness of AFLoRA.
AFLoRA freezes $\mathbf{A}$, effectively reducing both communication and computation costs by half. As training progresses, the client-specific ranks are adaptively adjusted and tend to decrease over time, leading to further reductions in resource consumption. When comparing the computation and communication overhead of AFLoRA, we observe that the introduction of the diagonal matrix significantly enhances representational capacity while incurring only negligible computational cost. This observation is also consistent with the results shown in Table~\ref{Table:domain}. 

In addition, \textbf{under IID scenario,} when tasks and data distributions are relatively uniform, AFLoRA’s design of freezing the shared matrix $\mathbf{A}$ on the client side reduces the instability of local updates and helps maintain a stable global representation, thereby improving convergence speed and final accuracy. The refinement mechanism further preserves domain-level common features across clients. 
\textbf{Under Non-IID scenario,} we set $\epsilon=0.5$. AFLoRA adapts the rank for each client based on its local data distribution, enabling better alignment with heterogeneous data. 
FLoRA requires transmitting stacked LoRA matrices, leading to high communication cost. 
HETLoRA performs zero-padding to match the maximum rank across clients, introducing a large number of ineffective parameters that dilute the aggregated updates and weaken generalization. 
FlexLoRA’s SVD decomposition not only incurs additional computational overhead but also introduces approximation errors.




\subsection{Evaluation on Domain Datasets}
We evaluate the model on the domain dataset to assess its adaptability to specific domains. In real-world scenarios, certain applications, such as finance and news recommendation, involving client data that is confined to a particular domain. We aim to verify whether the global model can effectively adapt to such domain-specific distributions. 

Table~\ref{Table:domain} presents the comparison between AFLoRA and baseline methods on the general dataset in terms of global model performance and computation/communication efficiency. The results show that AFLoRA consistently outperforms existing approaches.
\textbf{Under IID scenario,} when tasks and data distributions are relatively uniform, AFLoRA’s design of freezing the shared matrix $\mathbf{A}$ on the client side reduces the instability of local updates and helps maintain a stable global representation, thereby improving convergence speed and final accuracy. In domain-specific tasks with narrow focus, AFLoRA leverages its rank assignment mechanism to allocate limited resources to the most informative dimensions, enhancing overall performance. 
\textbf{Under Non-IID scenario,} AFLoRA adapts the rank for each client based on its local data distribution, enabling better alignment with heterogeneous data. Moreover, even on domain-specific datasets, refinement using public data can still enhance the generalization ability of the global model. It helps prevent the global model from overfitting to local client distributions and alleviates the impact of non-IID data.
FLoRA directly concatenates all $\mathbf{A}$ and $\mathbf{B}$ matrices, which in highly heterogeneous settings can cause the global model to be biased toward certain client distributions. 
HETLoRA suffers particularly from information dilution when padding is applied across clients with highly diverse ranks. 
FlexLoRA’s SVD-based reconstruction introduces errors that can significantly affect performance on heterogeneous clients.

\subsection{Performance under different non-IID degrees. }
We evaluate our method under varying degrees of data heterogeneity by setting $\epsilon=0.2, 0.4, 0.6$ for the Databricks-Dolly-15k dataset, with results presented in Fig.\ref{Table:performance-nonIID}.
Analysis of these results reveals several key findings. First, as $\epsilon$ increases, indicating reduced data skew across clients, we observe a consistent improvement in overall accuracy across all federated fine-tuning algorithms. 
Second, AFLoRA demonstrates remarkable stability, maintaining high accuracy levels across all $\epsilon$ settings. In contrast, baseline methods suffer substantial performance degradation under high data heterogeneity (low $\epsilon$ values), highlighting AFLoRA's robustness in non-IID scenarios.
Third, AFLoRA consistently outperforms competing approaches in both overall and generalization performance regardless of the degree of data heterogeneity. Notably, AFLoRA's advantages become increasingly pronounced as $\epsilon$ decreases. This can be attributed to the fact that higher data heterogeneity exacerbates the negative impact of uneven learning on the global model's generalization capabilities. While baseline methods struggle under these conditions, AFLoRA effectively mitigates such issues through its public data refinement step, resulting in significantly better performance, particularly in challenging non-IID environments.

==> rw-old.tex <==
\section{Related Work}\label{sec:related}
In this section, we first introduce the related work of FL with PEFT,  heterogeneous federated fine-tuning and accurate federated LoRA fine-tuning.

\subsection{Federated Learning with Parameter-Efficient Fine-Tuning}
%The large scale of foundation models, combined with the limited compute and bandwidth on edge devices, makes full-parameter federated fine-tuning impractical. 
%The enormous size of foundation models, while edge devices possess limited computational and communicational resources, makes full-parameter federated fine-tuning impractical.
%To address this, most FL approaches adopt PEFT, which updates only a small subset of parameters while preserving comparable downstream performance to full fine-tuning. 
The enormous size of foundation models and the limited resources of edge devices make full-parameter federated fine-tuning impractical, so most FL approaches adopt PEFT to update only a small subset of parameters while preserving comparable performance.
Representative methods include FedAdapter\cite{fedadapter} using adapter tuning which inserts small trainable adapters into selected layers, SLoRA\cite{slora} using LoRA tuning which applies low-rank decomposition to weight matrices, pFedprompt\cite{pFedPrompt} using prompt tuning which prepends learnable prompt tokens to the input, or FedPrefix\cite{fedperfix} using prefix tuning which tunes prefix vectors in the transformer layers. 
LoRA is arguably the most popular method among PEFT approaches, requiring the adjustment of less than 1\% of model parameters while achieving performance comparable to full fine-tuning across a wide range of tasks.



\subsection{Heterogeneous Federated Fine-Tuning}
Heterogeneity in resources such as computation, communication and data poses major challenges in FL, while existing solutions\cite{afl,fedprox,noniid1,noniid2} are often inadequate for LLMs. 
%To address resource heterogeneity, recent methods aim to support variable-rank or adaptive LoRA configurations, yet limitations remain. 
To address resource heterogeneity, recent methods support heterogeneous LoRA, but they either use fixed ranks throughout training which unable to adapt to changing learning state, or rely on heuristic strategies like arbitrary rank pruning rather than principled mechanisms, yet limitations remain.
FlexLoRA\cite{flexlora} and FLoRA\cite{flora} select the maximum rank based on local resources but keep it fixed and ignore the data distribution and varying local training state. 
%FLoRA\cite{flora} randomly assigns static ranks, failing to effectively adapt to the system and data resources of individual clients. 
HETLoRA\cite{hetlora} introduces rank self-pruning via regularization, but complex hyperparameter settings affect the performance. 
%HAFL\cite{hafl} selects only one row or column per update, reducing flexibility. 
PF2LoRA\cite{pf2lora} discards a fixed portion of LoRA parameters post-training, lacking adaptivity.
And AutoRank\cite{autorank} adjusts ranks via multi-factor analysis but is overly complex. 
These methods fall short in balancing efficiency, adaptability, and performance, highlighting the need for a lightweight and dynamic fine-tuning approach that can better adapt to the dynamic changes in the local model's learning progress on its data under heterogeneous and constrained resource.

\subsection{Accurate Federated LoRA Fine-Tuning}
%Building on the success of LoRA, several works\cite{openfedllm, fedsb} have explored integrating LoRA into FL. 
%A straightforward approach is to combine LoRA with the FedAvg\cite{fedavg} framework, as done in FedIT \cite{fedit}. 
%Based on this, variants such as SLoRA\cite{slora} use supervised fine-tuning to improve initialization, while FedSA-LoRA\cite{fedsalora} shares only the A matrix for aggregation to balance generalization and personalization. 
%FedLFC\cite{fedlfc} enables multilingual adaptation via clustering-based LoRA aggregation across language families.
Building on the success of LoRA, various works\cite{openfedllm, fedsb, fedsalora, fedlfc} have integrated it into FL system. 
Variants such as SLoRA\cite{slora}, FedSA-LoRA\cite{fedsalora}, and FedLFC\cite{fedlfc} improve LoRA-based FL by enhancing initialization, selectively aggregating parameters, or enabling multi-task adaptation through clustering.
Several studies have attempted to tackle this issue.
However, these methods often suffer from aggregation interference, the discrepancy between the averaged LoRA weights and locally updated ones, which can degrade global model performance. 
FlexLoRA\cite{flexlora} reconstructs full-rank LoRA weights via SVD, introducing extra computation and approximation error. 
FFA-LoRA\cite{ffalora} freezes A and fine-tunes only B, limiting representational capacity.
FLoRA\cite{flora} stacks LoRA matrices during aggregation, increasing communication cost.
Despite these efforts, none of the above approaches achieve accurate and efficient aggregation of heterogeneous LoRA adapters without sacrificing performance or scalability.
% 删掉或者加LoRA-A2 baseline
% BC顺序，
